A High-Precision NIR Survey for RV Variable Low-Mass Stars

We present the results of a precise near-infrared (NIR) radial velocity (RV) survey of 32 low-mass stars with spectral types K2-M4 using CSHELL at the NASA IRTF in the $K$-band with an isotopologue methane gas cell to achieve wavelength calibration and a novel iterative RV extraction method. We surveyed 14 members of young ($\approx$ 25-150 Myr) moving groups, the young field star $\varepsilon$ Eridani as well as 18 nearby ($<$ 25 pc) low-mass stars and achieved typical single-measurement precisions of 8-15 m s$^{-1}$ with a long-term stability of 15-50 m s$^{-1}$. We obtain the best NIR RV constraints to date on 27 targets in our sample, 19 of which were never followed by high-precision RV surveys. Our results indicate that very active stars can display long-term RV variations as low as $\sim$ 25-50 m s$^{-1}$ at $\approx$ 2.3125 $\mu$m, thus constraining the effect of jitter at these wavelengths. We provide the first multi-wavelength confirmation of GJ 876 bc and independently retrieve orbital parameters consistent with previous studies. We recovered RV variability for HD 160934 AB and GJ 725 AB that are consistent with their known binary orbits, and nine other targets are candidate RV variables with a statistical significance of 3-5$\sigma$. Our method combined with the new iSHELL spectrograph will yield long-term RV precisions of $\lesssim$ 5 m s$^{-1}$ in the NIR, which will allow the detection of Super-Earths near the habitable zone of mid-M dwarfs.

==> Table2_LONG.tex <==
% Observing log
\begin{deluxetable}{lccc}
\tablecolumns{4}
\tablecaption{Log of All Science Star Observations \label{tab:obslog}}
\tablehead{\colhead{Target} & \colhead{UT Date} & \colhead{Num. of} &  \colhead{Median}\\
\colhead{Name} & \colhead{(YYMMDD)} & \colhead{Spectra} & \colhead{S/N}}
\startdata
\textbf{AG~Tri} & 101009 & 6 & 23\\
& 101011 & 15 & 16\\
& 101012 & 12 & 23\\
& 101122 & 12 & 22\\
& 101123 & 12 & 26\\
& 101124 & 12 & 20\\
& 110216 & 9 & 22\\
& 110219 & 10 & 25\\
& 110716 & 10 & 20\\
& 110819 & 14 & 28\\
\hline\\[-6pt]
\textbf{AT~Mic~A} & 101010 & 6 & 39\\
& 101011 & 11 & 35\\
& 101013 & 10 & 28\\
& 101123 & 2 & 26\\
& 101124 & 6 & 43\\
& 110709 & 6 & 44\\
& 110714 & 6 & 40\\
& 110820 & 9 & 40\\
& 140706 & 9 & 48\\
\hline\\[-6pt]
\textbf{AT~Mic~B} & 101010 & 7 & 37\\
& 101011 & 6 & 35\\
& 101013 & 10 & 26\\
& 101124 & 6 & 44\\
& 110709 & 7 & 36\\
& 110714 & 11 & 29\\
& 110820 & 10 & 31\\
& 140917 & 26 & 39\\
& 141106 & 9 & 15\\
\hline\\[-6pt]
\textbf{AU~Mic} & 100916 & 5 & 38\\
& 101010 & 8 & 42\\
& 101011 & 10 & 33\\
& 101013 & 10 & 45\\
& 101123 & 6 & 45\\
& 110709 & 6 & 47\\
& 110712 & 12 & 31\\
& 110716 & 6 & 48\\
& 110818 & 3 & 74\\
& 110820 & 3 & 59\\
& 140706 & 8 & 75\\
& 140917 & 11 & 69\\
\hline\\[-6pt]
\textbf{BD+01~2447} & 101122 & 9 & 36\\
& 101123 & 7 & 36\\
& 101124 & 7 & 44\\
& 110216 & 6 & 41\\
& 110217 & 8 & 36\\
& 110218 & 8 & 50\\
& 110219 & 5 & 50\\
\hline\\[-6pt]
\textbf{BD--13~6424} & 101011 & 6 & 30\\
& 101122 & 12 & 28\\
& 101123 & 10 & 27\\
& 101124 & 13 & 26\\
& 110713 & 15 & 26\\
& 110716 & 18 & 18\\
& 110819 & 8 & 39\\
& 110820 & 9 & 34\\
\hline\\[-6pt]
\textbf{BD+20~1790} & 101011 & 5 & 22\\
& 101012 & 6 & 21\\
& 101122 & 9 & 29\\
& 101124 & 12 & 22\\
& 110216 & 3 & 16\\
& 110219 & 4 & 21\\
& 140414 & 33 & 18\\
& 140428 & 27 & 19\\
\hline\\[-6pt]
\textbf{$\epsilon$~Eri} & 100915 & 5 & 110\\
& 101009 & 20 & 68\\
& 101010 & 20 & 58\\
& 101011 & 20 & 71\\
& 101012 & 32 & 68\\
& 101122 & 20 & 73\\
& 101123 & 37 & 64\\
& 101124 & 40 & 59\\
& 110216 & 15 & 66\\
& 110217 & 10 & 66\\
& 110218 & 36 & 70\\
& 110710 & 10 & 49\\
& 110820 & 20 & 73\\
\hline\\[-6pt]
\textbf{EQ~Peg~A} & 110820 & 9 & 33\\
& 110821 & 5 & 49\\
& 120822 & 2 & 84\\
& 140917 & 20 & 49\\
& 141105 & 19 & 16\\
& 141119 & 25 & 38\\
& 141213 & 30 & 38\\
\hline\\[-6pt]
\textbf{EV~Lac} & 140604 & 22 & 57\\
& 140610 & 16 & 51\\
& 140619 & 21 & 44\\
& 140917 & 20 & 54\\
& 141214 & 38 & 26\\
\hline\\[-6pt]
\textbf{GJ~15~A} & 100915 & 1 & 92\\
& 100916 & 3 & 42\\
& 101009 & 4 & 75\\
& 101010 & 4 & 67\\
& 101011 & 6 & 37\\
& 101012 & 6 & 62\\
& 101013 & 9 & 54\\
& 101122 & 6 & 69\\
& 101123 & 4 & 66\\
& 101124 & 4 & 61\\
& 110710 & 6 & 48\\
& 110713 & 30 & 18\\
& 110820 & 10 & 37\\
& 110821 & 6 & 51\\
& 121211 & 4 & 48\\
\hline\\[-6pt]
\textbf{GJ~3305~AB} & 101009 & 6 & 21\\
& 101012 & 10 & 27\\
& 101124 & 13 & 27\\
& 110216 & 9 & 21\\
& 110218 & 10 & 32\\
\hline\\[-6pt]
\textbf{GJ~876} & 100915 & 3 & 57\\
& 100916 & 4 & 53\\
& 101009 & 3 & 56\\
& 101010 & 6 & 39\\
& 101011 & 6 & 40\\
& 101013 & 10 & 33\\
& 101122 & 8 & 51\\
& 101123 & 7 & 39\\
& 101124 & 8 & 40\\
& 110709 & 8 & 33\\
& 110710 & 8 & 35\\
& 110712 & 18 & 31\\
& 110716 & 12 & 31\\
& 110819 & 4 & 62\\
& 110820 & 3 & 60\\
& 110821 & 6 & 51\\
& 120822 & 3 & 78\\
\hline\\[-6pt]
\textbf{GJ~169} & 140917 & 20 & 57\\
& 141119 & 15 & 53\\
& 141213 & 25 & 52\\
& 141214 & 12 & 49\\
& 150125 & 35 & 35\\
\hline\\[-6pt]
\textbf{GJ~338~A} & 140311 & 16 & 53\\
& 140318 & 21 & 44\\
& 140319 & 11 & 65\\
& 140412 & 15 & 69\\
& 140429 & 17 & 51\\
& 141119 & 8 & 68\\
\hline\\[-6pt]
\textbf{GJ~338~B} & 140311 & 16 & 55\\
& 140319 & 13 & 60\\
& 140412 & 15 & 67\\
& 140414 & 20 & 47\\
& 140429 & 16 & 53\\
& 141119 & 8 & 77\\
& 150125 & 4 & 24\\
\hline\\[-6pt]
\textbf{GJ~3942} & 140319 & 44 & 22\\
& 140411 & 4 & 20\\
& 140417 & 29 & 25\\
& 140422 & 64 & 21\\
& 140429 & 30 & 28\\
& 140610 & 38 & 31\\
& 140619 & 45 & 29\\
\hline\\[-6pt]
%\textbf{GJ~411} & 140305 & 21 & 39\\
%& 140316 & 7 & 89\\
%& 140319 & 8 & 74\\
%\hline\\[-6pt]
\textbf{GJ~458~A} & 140311 & 47 & 25\\
& 140319 & 51 & 25\\
& 140411 & 37 & 29\\
& 140413 & 43 & 30\\
& 140428 & 21 & 18\\
& 140618 & 35 & 34\\
& 140619 & 40 & 31\\
\hline\\[-6pt]
\textbf{GJ~537~A} & 140306 & 60 & 25\\
& 140311 & 45 & 26\\
& 140320 & 35 & 24\\
& 140413 & 25 & 28\\
& 140422 & 17 & 23\\
& 140507 & 30 & 33\\
& 140508 & 28 & 30\\
& 140519 & 28 & 39\\
& 140520 & 41 & 25\\
& 140604 & 14 & 30\\
\hline\\[-6pt]
\textbf{GJ~537~B} & 140305 & 51 & 19\\
& 140318 & 16 & 21\\
& 140320 & 33 & 32\\
& 140411 & 26 & 32\\
& 140429 & 30 & 36\\
& 140519 & 37 & 38\\
& 140618 & 39 & 37\\
& 150125 & 26 & 27\\
\hline\\[-6pt]
%\textbf{GJ~654} & 140508 & 30 & 25\\
%& 140608 & 30 & 28\\
%& 140618 & 30 & 36\\
%\hline\\[-6pt]
\textbf{GJ~725~A} & 110819 & 7 & 39\\
& 110820 & 6 & 50\\
& 110821 & 8 & 49\\
& 140618 & 19 & 55\\
& 140619 & 13 & 59\\
\hline\\[-6pt]
\textbf{GJ~740} & 140306 & 30 & 31\\
& 140316 & 20 & 32\\
& 140321 & 33 & 41\\
& 140421 & 15 & 25\\
& 140427 & 27 & 24\\
& 140507 & 30 & 45\\
& 140604 & 23 & 42\\
& 140608 & 31 & 44\\
& 140610 & 10 & 42\\
& 140619 & 21 & 44\\
& 140707 & 35 & 37\\
\hline\\[-6pt]
\textbf{GJ~9520} & 140317 & 30 & 42\\
& 140321 & 42 & 27\\
& 140411 & 23 & 40\\
& 140414 & 58 & 28\\
& 140420 & 16 & 24\\
& 140428 & 25 & 20\\
& 150125 & 44 & 26\\
\hline\\[-6pt]
\textbf{HD~160934~AB} & 100916 & 5 & 18\\
& 101013 & 12 & 19\\
& 110709 & 8 & 26\\
& 110713 & 10 & 18\\
& 110820 & 12 & 31\\
\hline\\[-6pt]
\textbf{LHS~26} & 140917 & 22 & 43\\
& 141106 & 33 & 19\\
& 141119 & 40 & 25\\
& 150125 & 45 & 31\\
& 150131 & 40 & 26\\
\hline\\[-6pt]
\textbf{LHS~371} & 140310 & 37 & 28\\
& 140319 & 42 & 27\\
& 140320 & 33 & 34\\
& 140412 & 29 & 30\\
& 140417 & 34 & 32\\
\hline\\[-6pt]
\textbf{LHS~372} & 140311 & 38 & 23\\
& 140317 & 28 & 31\\
& 140427 & 7 & 22\\
& 140429 & 33 & 25\\
\hline\\[-6pt]
\textbf{LHS~374} & 140307 & 30 & 37\\
& 140316 & 51 & 29\\
& 140319 & 43 & 27\\
& 140412 & 41 & 30\\
& 140419 & 34 & 25\\
\hline\\[-6pt]
\textbf{LO~Peg} & 101009 & 4 & 31\\
& 101010 & 6 & 23\\
& 101011 & 6 & 32\\
& 101013 & 14 & 19\\
& 101123 & 14 & 24\\
& 101124 & 12 & 26\\
& 110710 & 4 & 25\\
& 110713 & 9 & 34\\
& 110714 & 18 & 22\\
& 110819 & 15 & 27\\
\hline\\[-6pt]
\textbf{TYC~5899--26--1} & 101012 & 9 & 23\\
& 101122 & 11 & 29\\
& 101123 & 12 & 28\\
& 101124 & 11 & 27\\
& 110219 & 8 & 31\\
\hline\\[-6pt]
\textbf{V1005~Ori} & 101010 & 6 & 28\\
& 101012 & 10 & 29\\
& 101122 & 10 & 31\\
& 101123 & 14 & 27\\
& 101124 & 11 & 28\\
& 110216 & 6 & 34\\
& 110218 & 8 & 44\\
\hline\\[-6pt]
\textbf{V577~Per} & 100916 & 2 & 36\\
& 101011 & 10 & 23\\
& 101122 & 10 & 29\\
& 101123 & 19 & 24\\
& 110215 & 9 & 30\\
& 110220 & 11 & 22\\
& 110714 & 11 & 25\\
& 110819 & 14 & 33\\
& 110820 & 8 & 40\\[-7pt]
\enddata
\tablecomments{See Section~\ref{sec:obs} for more details.}
\end{deluxetable}

==> Table3_LONG.tex <==
% Detailed RVs
\begin{deluxetable}{lr@{\hspace{1pt}}c@{\hspace{1pt}}lr@{\hspace{1pt}}c@{\hspace{1pt}}lc}
\tablecolumns{8}
\tablecaption{Detailed Radial Velocity Measurements \label{tab:detrv}}
\tablehead{\colhead{Target} & \multicolumn{3}{c}{Red. Julian Date} & \multicolumn{3}{c}{Relative} & \colhead{\added{S/N}}\\
\colhead{Name} & \multicolumn{3}{c}{JD$-2400000$} & \multicolumn{3}{c}{RV (\ms)} & \colhead{Ratio}}
\startdata
\textbf{AG Tri} & 55479.003 & $ \pm $ & 0.003 & \hphantom{3pt}107 & $ \pm $ & 51 & 23\hphantom{3pt}\\
& 55480.930 & $ \pm $ & 0.004 & \hphantom{3pt}-139 & $ \pm $ & 50 & 16\hphantom{3pt}\\
& 55482.015 & $ \pm $ & 0.006 & \hphantom{3pt}10 & $ \pm $ & 27 & 23\hphantom{3pt}\\
& 55522.875 & $ \pm $ & 0.003 & \hphantom{3pt}198 & $ \pm $ & 43 & 22\hphantom{3pt}\\
& 55523.855 & $ \pm $ & 0.003 & \hphantom{3pt}76 & $ \pm $ & 45 & 26\hphantom{3pt}\\
& 55524.871 & $ \pm $ & 0.003 & \hphantom{3pt}-76 & $ \pm $ & 77 & 20\hphantom{3pt}\\
& 55608.734 & $ \pm $ & 0.004 & \hphantom{3pt}64 & $ \pm $ & 103 & 22\hphantom{3pt}\\
& 55611.739 & $ \pm $ & 0.003 & \hphantom{3pt}29 & $ \pm $ & 50 & 25\hphantom{3pt}\\
& 55759.126 & $ \pm $ & 0.004 & \hphantom{3pt}26 & $ \pm $ & 48 & 20\hphantom{3pt}\\
& 55793.018 & $ \pm $ & 0.004 & \hphantom{3pt}-77 & $ \pm $ & 22 & 28\hphantom{3pt}\\
\hline\\[-6pt]
\textbf{AT Mic A} & 55479.735 & $ \pm $ & 0.001 & 34 & $ \pm $ & 25 & 39\\
& 55480.729 & $ \pm $ & 0.004 & 0 & $ \pm $ & 40 & 35\\
& 55482.776 & $ \pm $ & 0.001 & -15 & $ \pm $ & 59 & 28\\
& 55523.713 & $ \pm $ & 0.001 & -97 & $ \pm $ & 118 & 26\\
& 55524.702 & $ \pm $ & 0.002 & 7 & $ \pm $ & 31 & 43\\
& 55752.045 & $ \pm $ & 0.002 & -44 & $ \pm $ & 22 & 44\\
& 55756.968 & $ \pm $ & 0.002 & -84 & $ \pm $ & 63 & 40\\
& 55793.851 & $ \pm $ & 0.002 & -15 & $ \pm $ & 22 & 40\\
& 56844.995 & $ \pm $ & 0.002 & 49 & $ \pm $ & 23 & 48\\
\hline\\[-6pt]
\textbf{AT Mic B} & 55479.717 & $ \pm $ & 0.001 & 80 & $ \pm $ & 68 & 37\\
& 55480.751 & $ \pm $ & 0.002 & 140 & $ \pm $ & 66 & 35\\
& 55482.793 & $ \pm $ & 0.001 & 8 & $ \pm $ & 74 & 26\\
& 55524.726 & $ \pm $ & 0.002 & 32 & $ \pm $ & 58 & 44\\
& 55752.073 & $ \pm $ & 0.003 & -294 & $ \pm $ & 97 & 36\\
& 55756.996 & $ \pm $ & 0.003 & -47 & $ \pm $ & 113 & 29\\
& 55793.875 & $ \pm $ & 0.002 & -13 & $ \pm $ & 45 & 31\\
& 56917.841 & $ \pm $ & 0.009 & -73 & $ \pm $ & 48 & 39\\
& 56967.774 & $ \pm $ & 0.007 & 508 & $ \pm $ & 203 & 15\\
\hline\\[-6pt]
\textbf{AU Mic} & 55455.854 & $ \pm $ & 0.002 & 83 & $ \pm $ & 108 & 38\\
& 55479.800 & $ \pm $ & 0.001 & 8 & $ \pm $ & 22 & 42\\
& 55480.769 & $ \pm $ & 0.001 & 73 & $ \pm $ & 55 & 33\\
& 55482.756 & $ \pm $ & 0.001 & 51 & $ \pm $ & 30 & 45\\
& 55523.700 & $ \pm $ & 0.001 & -2 & $ \pm $ & 23 & 45\\
& 55752.100 & $ \pm $ & 0.002 & -42 & $ \pm $ & 39 & 47\\
& 55755.077 & $ \pm $ & 0.002 & 52 & $ \pm $ & 45 & 31\\
& 55758.968 & $ \pm $ & 0.002 & -122 & $ \pm $ & 31 & 48\\
& 55791.814 & $ \pm $ & 0.001 & 31 & $ \pm $ & 51 & 74\\
& 55793.832 & $ \pm $ & 0.001 & 61 & $ \pm $ & 8 & 59\\
& 56844.960 & $ \pm $ & 0.002 & -42 & $ \pm $ & 14 & 75\\
& 56917.743 & $ \pm $ & 0.002 & -24 & $ \pm $ & 18 & 69\\
\hline\\[-6pt]
\textbf{BD+01 2447} & 55523.147 & $ \pm $ & 0.002 & -36 & $ \pm $ & 31 & 36\\
& 55524.130 & $ \pm $ & 0.002 & -27 & $ \pm $ & 32 & 36\\
& 55525.112 & $ \pm $ & 0.006 & 11 & $ \pm $ & 27 & 44\\
& 55608.892 & $ \pm $ & 0.001 & -30 & $ \pm $ & 21 & 41\\
& 55609.888 & $ \pm $ & 0.002 & 24 & $ \pm $ & 23 & 36\\
& 55610.909 & $ \pm $ & 0.002 & 11 & $ \pm $ & 14 & 50\\
& 55611.887 & $ \pm $ & 0.002 & 14 & $ \pm $ & 24 & 50\\
\hline\\[-6pt]
\textbf{BD--13 6424} & 55480.843 & $ \pm $ & 0.002 & 95 & $ \pm $ & 64 & 30\\
& 55522.796 & $ \pm $ & 0.003 & -60 & $ \pm $ & 41 & 28\\
& 55523.778 & $ \pm $ & 0.002 & 76 & $ \pm $ & 39 & 27\\
& 55524.805 & $ \pm $ & 0.002 & 109 & $ \pm $ & 37 & 26\\
& 55756.103 & $ \pm $ & 0.004 & 14 & $ \pm $ & 47 & 26\\
& 55759.057 & $ \pm $ & 0.004 & -237 & $ \pm $ & 63 & 18\\
& 55792.973 & $ \pm $ & 0.003 & 113 & $ \pm $ & 36 & 39\\
& 55794.013 & $ \pm $ & 0.003 & -37 & $ \pm $ & 16 & 34\\
\hline\\[-6pt]
\textbf{BD+20 1790} & 55481.144 & $ \pm $ & 0.003 & -201 & $ \pm $ & 171 & 22\\
& 55482.157 & $ \pm $ & 0.002 & 620 & $ \pm $ & 78 & 21\\
& 55523.081 & $ \pm $ & 0.004 & 76 & $ \pm $ & 50 & 29\\
& 55525.056 & $ \pm $ & 0.003 & -100 & $ \pm $ & 45 & 22\\
& 55608.918 & $ \pm $ & 0.001 & 562 & $ \pm $ & 334 & 16\\
& 55611.821 & $ \pm $ & 0.003 & 592 & $ \pm $ & 218 & 21\\
& 56761.754 & $ \pm $ & 0.004 & -654 & $ \pm $ & 79 & 18\\
& 56775.799 & $ \pm $ & 0.004 & 82 & $ \pm $ & 90 & 19\\
\hline\\[-6pt]
\textbf{$\epsilon$ Eri} & 55455.093 & $ \pm $ & 0.001 & -26 & $ \pm $ & 18 & 110\\
& 55479.144 & $ \pm $ & 0.000 & 8 & $ \pm $ & 12 & 68\\
& 55480.001 & $ \pm $ & 0.000 & 12 & $ \pm $ & 16 & 58\\
& 55481.056 & $ \pm $ & 0.000 & 4 & $ \pm $ & 11 & 71\\
& 55482.016 & $ \pm $ & 0.000 & -19 & $ \pm $ & 14 & 68\\
& 55522.920 & $ \pm $ & 0.000 & 42 & $ \pm $ & 11 & 73\\
& 55523.886 & $ \pm $ & 0.000 & 33 & $ \pm $ & 8 & 64\\
& 55524.954 & $ \pm $ & 0.000 & 38 & $ \pm $ & 10 & 59\\
& 55608.764 & $ \pm $ & 0.000 & -29 & $ \pm $ & 15 & 66\\
& 55609.788 & $ \pm $ & 0.000 & 2 & $ \pm $ & 22 & 66\\
& 55610.792 & $ \pm $ & 0.001 & -14 & $ \pm $ & 10 & 70\\
& 55753.102 & $ \pm $ & 0.001 & -102 & $ \pm $ & 29 & 49\\
& 55794.090 & $ \pm $ & 0.000 & -29 & $ \pm $ & 12 & 73\\
\hline\\[-6pt]
\textbf{EQ Peg A} & 55793.979 & $ \pm $ & 0.002 & -225 & $ \pm $ & 102 & 33\\
& 55794.961 & $ \pm $ & 0.002 & -7 & $ \pm $ & 29 & 49\\
& 56917.939 & $ \pm $ & 0.003 & -105 & $ \pm $ & 23 & 84\\
& 56966.884 & $ \pm $ & 0.004 & -605 & $ \pm $ & 245 & 49\\
& 56980.888 & $ \pm $ & 0.003 & 282 & $ \pm $ & 34 & 16\\
\hline\\[-6pt]
\textbf{EV Lac} & 56813.126 & $ \pm $ & 0.003 & 2 & $ \pm $ & 14 & 57\\
& 56819.085 & $ \pm $ & 0.003 & 20 & $ \pm $ & 13 & 51\\
& 56828.117 & $ \pm $ & 0.003 & 25 & $ \pm $ & 16 & 44\\
& 56918.000 & $ \pm $ & 0.003 & -71 & $ \pm $ & 9 & 54\\
& 57005.794 & $ \pm $ & 0.005 & 76 & $ \pm $ & 25 & 26\\
\hline\\[-6pt]
\textbf{GJ 15 A} & 55455.833 & $ \pm $ & 0.001 & -58 & $ \pm $ & 61 & 92\\
& 55478.960 & $ \pm $ & 0.001 & -19 & $ \pm $ & 9 & 42\\
& 55479.986 & $ \pm $ & 0.002 & 12 & $ \pm $ & 11 & 75\\
& 55480.869 & $ \pm $ & 0.001 & -24 & $ \pm $ & 31 & 67\\
& 55481.968 & $ \pm $ & 0.001 & -15 & $ \pm $ & 19 & 37\\
& 55482.867 & $ \pm $ & 0.001 & -8 & $ \pm $ & 16 & 62\\
& 55522.908 & $ \pm $ & 0.001 & -4 & $ \pm $ & 20 & 54\\
& 55523.826 & $ \pm $ & 0.001 & -29 & $ \pm $ & 17 & 69\\
& 55524.838 & $ \pm $ & 0.001 & 20 & $ \pm $ & 20 & 66\\
& 55753.040 & $ \pm $ & 0.003 & -47 & $ \pm $ & 44 & 61\\
& 55756.151 & $ \pm $ & 0.001 & 112 & $ \pm $ & 31 & 48\\
& 55794.045 & $ \pm $ & 0.001 & 20 & $ \pm $ & 25 & 18\\
& 55794.976 & $ \pm $ & 0.001 & 8 & $ \pm $ & 17 & 37\\
& 56272.876 & $ \pm $ & 0.001 & 11 & $ \pm $ & 10 & 51\\
\hline\\[-6pt]
\textbf{GJ 3305} & 55479.131 & $ \pm $ & 0.001 & -202 & $ \pm $ & 78 & 21\\
& 55482.077 & $ \pm $ & 0.002 & -46 & $ \pm $ & 44 & 27\\
& 55608.824 & $ \pm $ & 0.003 & 144 & $ \pm $ & 102 & 21\\
& 55610.870 & $ \pm $ & 0.003 & 60 & $ \pm $ & 37 & 32\\
\hline\\[-6pt]
\textbf{GJ 876} & 55454.990 & $ \pm $ & 0.004 & -302 & $ \pm $ & 31 & 57\\
& 55455.997 & $ \pm $ & 0.004 & -278 & $ \pm $ & 28 & 53\\
& 55478.861 & $ \pm $ & 0.001 & 211 & $ \pm $ & 33 & 56\\
& 55479.927 & $ \pm $ & 0.002 & 172 & $ \pm $ & 19 & 39\\
& 55480.822 & $ \pm $ & 0.002 & 216 & $ \pm $ & 20 & 40\\
& 55482.816 & $ \pm $ & 0.001 & 172 & $ \pm $ & 33 & 33\\
& 55522.731 & $ \pm $ & 0.004 & -35 & $ \pm $ & 8 & 51\\
& 55523.799 & $ \pm $ & 0.001 & 4 & $ \pm $ & 18 & 39\\
& 55524.779 & $ \pm $ & 0.001 & 64 & $ \pm $ & 16 & 40\\
& 55752.134 & $ \pm $ & 0.001 & -316 & $ \pm $ & 22 & 33\\
& 55753.076 & $ \pm $ & 0.003 & -646 & $ \pm $ & 41 & 35\\
& 55755.127 & $ \pm $ & 0.003 & -466 & $ \pm $ & 23 & 31\\
& 55759.006 & $ \pm $ & 0.003 & -373 & $ \pm $ & 26 & 31\\
& 55792.950 & $ \pm $ & 0.001 & 102 & $ \pm $ & 10 & 62\\
& 55793.957 & $ \pm $ & 0.001 & 63 & $ \pm $ & 18 & 60\\
& 55794.936 & $ \pm $ & 0.002 & 117 & $ \pm $ & 14 & 51\\
& 56161.968 & $ \pm $ & 0.002 & 95 & $ \pm $ & 7 & 78\\
\hline\\[-6pt]
\textbf{GJ 169} & 56918.066 & $ \pm $ & 0.003 & -10 & $ \pm $ & 12 & 57\\
& 56980.957 & $ \pm $ & 0.003 & -35 & $ \pm $ & 14 & 53\\
& 57004.878 & $ \pm $ & 0.003 & 20 & $ \pm $ & 11 & 52\\
& 57005.881 & $ \pm $ & 0.007 & -18 & $ \pm $ & 18 & 49\\
& 57047.892 & $ \pm $ & 0.004 & 38 & $ \pm $ & 14 & 35\\
\hline\\[-6pt]
\textbf{GJ 338 A} & 56727.884 & $ \pm $ & 0.007 & 13 & $ \pm $ & 9 & 53\\
& 56734.898 & $ \pm $ & 0.004 & -34 & $ \pm $ & 13 & 44\\
& 56735.767 & $ \pm $ & 0.002 & -16 & $ \pm $ & 18 & 65\\
& 56759.849 & $ \pm $ & 0.003 & -12 & $ \pm $ & 10 & 69\\
& 56776.773 & $ \pm $ & 0.002 & 14 & $ \pm $ & 10 & 51\\
& 56981.103 & $ \pm $ & 0.002 & 30 & $ \pm $ & 15 & 68\\
\hline\\[-6pt]
\textbf{GJ 338 B} & 56727.893 & $ \pm $ & 0.002 & 22 & $ \pm $ & 6 & 55\\
& 56735.741 & $ \pm $ & 0.002 & -19 & $ \pm $ & 7 & 60\\
& 56759.793 & $ \pm $ & 0.002 & -1 & $ \pm $ & 14 & 67\\
& 56761.839 & $ \pm $ & 0.004 & -72 & $ \pm $ & 18 & 47\\
& 56776.821 & $ \pm $ & 0.001 & 60 & $ \pm $ & 12 & 53\\
& 56981.136 & $ \pm $ & 0.002 & -10 & $ \pm $ & 10 & 77\\
\hline\\[-6pt]
\textbf{GJ 3942} & 56736.117 & $ \pm $ & 0.004 & 151 & $ \pm $ & 34 & 22\\
& 56759.064 & $ \pm $ & 0.001 & 158 & $ \pm $ & 138 & 20\\
& 56765.116 & $ \pm $ & 0.004 & -85 & $ \pm $ & 24 & 25\\
& 56770.063 & $ \pm $ & 0.006 & -103 & $ \pm $ & 25 & 21\\
& 56777.099 & $ \pm $ & 0.004 & -101 & $ \pm $ & 27 & 28\\
& 56819.004 & $ \pm $ & 0.004 & 80 & $ \pm $ & 14 & 31\\
& 56827.917 & $ \pm $ & 0.004 & -10 & $ \pm $ & 14 & 29\\
\hline\\[-6pt]
\textbf{GJ 411} & 56722.027 & $ \pm $ & 0.002 & 23 & $ \pm $ & 21 & 39\\
& 56732.945 & $ \pm $ & 0.001 & -37 & $ \pm $ & 1 & 89\\
& 56735.789 & $ \pm $ & 0.001 & 24 & $ \pm $ & 12 & 74\\
\hline\\[-6pt]
\textbf{GJ 458 A} & 56728.060 & $ \pm $ & 0.003 & 50 & $ \pm $ & 14 & 25\\
& 56735.854 & $ \pm $ & 0.004 & -5 & $ \pm $ & 15 & 25\\
& 56758.938 & $ \pm $ & 0.004 & 27 & $ \pm $ & 17 & 29\\
& 56760.960 & $ \pm $ & 0.004 & -25 & $ \pm $ & 14 & 30\\
& 56775.930 & $ \pm $ & 0.007 & 48 & $ \pm $ & 35 & 18\\
& 56826.818 & $ \pm $ & 0.004 & -30 & $ \pm $ & 14 & 34\\
& 56827.793 & $ \pm $ & 0.004 & -22 & $ \pm $ & 13 & 31\\
\hline\\[-6pt]
\textbf{GJ 537 A} & 56723.031 & $ \pm $ & 0.003 & -70 & $ \pm $ & 20 & 25\\
& 56727.971 & $ \pm $ & 0.003 & 53 & $ \pm $ & 20 & 26\\
& 56736.961 & $ \pm $ & 0.005 & 91 & $ \pm $ & 35 & 24\\
& 56761.052 & $ \pm $ & 0.004 & -111 & $ \pm $ & 25 & 28\\
& 56769.947 & $ \pm $ & 0.003 & -14 & $ \pm $ & 63 & 23\\
& 56785.009 & $ \pm $ & 0.005 & -10 & $ \pm $ & 24 & 33\\
& 56786.020 & $ \pm $ & 0.003 & 32 & $ \pm $ & 20 & 30\\
& 56796.777 & $ \pm $ & 0.003 & 8 & $ \pm $ & 14 & 39\\
& 56797.791 & $ \pm $ & 0.004 & 30 & $ \pm $ & 26 & 25\\
& 56812.994 & $ \pm $ & 0.004 & 80 & $ \pm $ & 67 & 30\\
\hline\\[-6pt]
\textbf{GJ 537 B} & 56722.114 & $ \pm $ & 0.005 & -74 & $ \pm $ & 41 & 19\\
& 56735.096 & $ \pm $ & 0.006 & 141 & $ \pm $ & 51 & 21\\
& 56737.041 & $ \pm $ & 0.004 & 19 & $ \pm $ & 17 & 32\\
& 56759.112 & $ \pm $ & 0.004 & -8 & $ \pm $ & 19 & 32\\
& 56776.926 & $ \pm $ & 0.004 & -155 & $ \pm $ & 19 & 36\\
& 56796.866 & $ \pm $ & 0.004 & 12 & $ \pm $ & 10 & 38\\
& 56826.929 & $ \pm $ & 0.004 & 83 & $ \pm $ & 17 & 37\\
& 57048.002 & $ \pm $ & 0.003 & 29 & $ \pm $ & 30 & 27\\
\hline\\[-6pt]
\textbf{GJ 654} & 56786.113 & $ \pm $ & 0.004 & -55 & $ \pm $ & 26 & 25\\
& 56817.020 & $ \pm $ & 0.004 & -56 & $ \pm $ & 18 & 28\\
& 56827.041 & $ \pm $ & 0.004 & 57 & $ \pm $ & 12 & 36\\
\hline\\[-6pt]
\textbf{GJ 725 A} & 55792.877 & $ \pm $ & 0.001 & -91 & $ \pm $ & 23 & 39\\
& 55793.901 & $ \pm $ & 0.002 & -35 & $ \pm $ & 11 & 50\\
& 55794.745 & $ \pm $ & 0.004 & -71 & $ \pm $ & 22 & 49\\
& 56827.119 & $ \pm $ & 0.003 & 65 & $ \pm $ & 11 & 55\\
& 56828.065 & $ \pm $ & 0.003 & 43 & $ \pm $ & 7 & 59\\
\hline\\[-6pt]
\textbf{GJ 740} & 56723.142 & $ \pm $ & 0.003 & 54 & $ \pm $ & 19 & 31\\
& 56733.157 & $ \pm $ & 0.002 & 173 & $ \pm $ & 23 & 32\\
& 56738.129 & $ \pm $ & 0.004 & 67 & $ \pm $ & 14 & 41\\
& 56769.036 & $ \pm $ & 0.003 & 59 & $ \pm $ & 35 & 25\\
& 56775.121 & $ \pm $ & 0.003 & -51 & $ \pm $ & 19 & 24\\
& 56785.107 & $ \pm $ & 0.004 & 26 & $ \pm $ & 12 & 45\\
& 56813.063 & $ \pm $ & 0.003 & 23 & $ \pm $ & 10 & 42\\
& 56817.104 & $ \pm $ & 0.004 & -14 & $ \pm $ & 10 & 44\\
& 56819.129 & $ \pm $ & 0.002 & -97 & $ \pm $ & 18 & 42\\
& 56828.009 & $ \pm $ & 0.003 & -95 & $ \pm $ & 15 & 44\\
& 56845.969 & $ \pm $ & 0.004 & -27 & $ \pm $ & 13 & 37\\
\hline\\[-6pt]
\textbf{GJ 9520} & 56734.062 & $ \pm $ & 0.004 & 51 & $ \pm $ & 13 & 42\\
& 56738.037 & $ \pm $ & 0.004 & -77 & $ \pm $ & 19 & 27\\
& 56759.024 & $ \pm $ & 0.003 & 41 & $ \pm $ & 16 & 40\\
& 56762.064 & $ \pm $ & 0.005 & -161 & $ \pm $ & 23 & 28\\
& 56767.964 & $ \pm $ & 0.006 & -38 & $ \pm $ & 78 & 24\\
& 56776.092 & $ \pm $ & 0.009 & -77 & $ \pm $ & 43 & 20\\
& 57048.117 & $ \pm $ & 0.004 & 78 & $ \pm $ & 20 & 26\\
\hline\\[-6pt]
\textbf{HD 160934} & 55455.790 & $ \pm $ & 0.002 & 2359 & $ \pm $ & 635 & 18\\
& 55482.710 & $ \pm $ & 0.002 & 1190 & $ \pm $ & 130 & 19\\
& 55751.991 & $ \pm $ & 0.003 & 205 & $ \pm $ & 164 & 26\\
& 55755.981 & $ \pm $ & 0.005 & 555 & $ \pm $ & 127 & 18\\
& 55793.780 & $ \pm $ & 0.004 & -381 & $ \pm $ & 57 & 31\\
\hline\\[-6pt]
\textbf{LHS 26} & 56918.130 & $ \pm $ & 0.003 & 12 & $ \pm $ & 10 & 43\\
& 56967.869 & $ \pm $ & 0.004 & 37 & $ \pm $ & 34 & 19\\
& 56981.033 & $ \pm $ & 0.004 & 28 & $ \pm $ & 14 & 25\\
& 57047.784 & $ \pm $ & 0.005 & -21 & $ \pm $ & 15 & 31\\
& 57053.789 & $ \pm $ & 0.004 & -27 & $ \pm $ & 14 & 26\\
\hline\\[-6pt]
\textbf{LHS 371} & 56727.132 & $ \pm $ & 0.004 & 59 & $ \pm $ & 17 & 28\\
& 56735.945 & $ \pm $ & 0.003 & -91 & $ \pm $ & 19 & 27\\
& 56737.125 & $ \pm $ & 0.004 & -25 & $ \pm $ & 10 & 34\\
& 56759.969 & $ \pm $ & 0.005 & 50 & $ \pm $ & 19 & 30\\
& 56765.022 & $ \pm $ & 0.004 & 6 & $ \pm $ & 15 & 32\\
\hline\\[-6pt]
\textbf{LHS 372} & 56728.148 & $ \pm $ & 0.003 & 67 & $ \pm $ & 20 & 23\\
& 56734.126 & $ \pm $ & 0.004 & -61 & $ \pm $ & 14 & 31\\
& 56775.040 & $ \pm $ & 0.001 & -94 & $ \pm $ & 76 & 22\\
& 56777.012 & $ \pm $ & 0.004 & 51 & $ \pm $ & 21 & 25\\
\hline\\[-6pt]
\textbf{LHS 374} & 56724.044 & $ \pm $ & 0.004 & -28 & $ \pm $ & 12 & 37\\
& 56733.010 & $ \pm $ & 0.004 & 63 & $ \pm $ & 13 & 29\\
& 56736.018 & $ \pm $ & 0.003 & 56 & $ \pm $ & 15 & 27\\
& 56760.118 & $ \pm $ & 0.004 & -91 & $ \pm $ & 19 & 30\\
& 56767.019 & $ \pm $ & 0.010 & -259 & $ \pm $ & 40 & 25\\
\hline\\[-6pt]
\textbf{LO Peg} & 55478.923 & $ \pm $ & 0.002 & -449 & $ \pm $ & 550 & 31\\
& 55479.877 & $ \pm $ & 0.002 & -389 & $ \pm $ & 157 & 23\\
& 55480.801 & $ \pm $ & 0.002 & -551 & $ \pm $ & 448 & 32\\
& 55482.895 & $ \pm $ & 0.002 & -950 & $ \pm $ & 1675 & 19\\
& 55523.745 & $ \pm $ & 0.003 & -1491 & $ \pm $ & 287 & 24\\
& 55524.753 & $ \pm $ & 0.002 & -431 & $ \pm $ & 127 & 26\\
& 55752.967 & $ \pm $ & 0.002 & 1955 & $ \pm $ & 118 & 25\\
& 55756.051 & $ \pm $ & 0.003 & 3 & $ \pm $ & 60 & 34\\
& 55757.068 & $ \pm $ & 0.005 & -787 & $ \pm $ & 127 & 22\\
& 55792.927 & $ \pm $ & 0.002 & -307 & $ \pm $ & 104 & 27\\
\hline\\[-6pt]
\textbf{LP 776----25} & 55482.136 & $ \pm $ & 0.002 & 70 & $ \pm $ & 57 & 23\\
& 55522.971 & $ \pm $ & 0.004 & 24 & $ \pm $ & 33 & 29\\
& 55523.977 & $ \pm $ & 0.004 & -28 & $ \pm $ & 26 & 28\\
& 55525.008 & $ \pm $ & 0.003 & -40 & $ \pm $ & 43 & 27\\
& 55611.786 & $ \pm $ & 0.003 & 7 & $ \pm $ & 20 & 31\\
\hline\\[-6pt]
\textbf{V1005 Ori} & 55480.053 & $ \pm $ & 0.002 & -126 & $ \pm $ & 120 & 28\\
& 55482.102 & $ \pm $ & 0.002 & -67 & $ \pm $ & 54 & 29\\
& 55523.042 & $ \pm $ & 0.002 & 18 & $ \pm $ & 54 & 31\\
& 55524.087 & $ \pm $ & 0.004 & -72 & $ \pm $ & 62 & 27\\
& 55524.973 & $ \pm $ & 0.002 & -56 & $ \pm $ & 47 & 28\\
& 55608.862 & $ \pm $ & 0.002 & 92 & $ \pm $ & 61 & 34\\
& 55610.820 & $ \pm $ & 0.003 & 21 & $ \pm $ & 22 & 44\\
\hline\\[-6pt]
\textbf{V577 Per} & 55456.078 & $ \pm $ & 0.003 & -63 & $ \pm $ & 57 & 36\\
& 55481.081 & $ \pm $ & 0.002 & 184 & $ \pm $ & 87 & 23\\
& 55523.011 & $ \pm $ & 0.002 & 16 & $ \pm $ & 68 & 29\\
& 55523.918 & $ \pm $ & 0.003 & 378 & $ \pm $ & 104 & 24\\
& 55607.868 & $ \pm $ & 0.003 & 483 & $ \pm $ & 130 & 30\\
& 55612.720 & $ \pm $ & 0.006 & -338 & $ \pm $ & 303 & 22\\
& 55757.129 & $ \pm $ & 0.003 & 372 & $ \pm $ & 231 & 25\\
& 55793.078 & $ \pm $ & 0.004 & -335 & $ \pm $ & 99 & 33\\
& 55794.068 & $ \pm $ & 0.003 & -466 & $ \pm $ & 107 & 40\\

\enddata
\tablecomments{See Section~\ref{sec:results} for more details.}
\end{deluxetable}
